Lepton universality violation in the MF331 model

We perform a detailed study of the $\text{b} \to \text{c} \tau \nu$ and $\text{b} \to \text{s} l^+ l^-$ processes in a minimal flipped 331 model based on the $SU(3)_C\times SU(3)_L\times U(1)_N$ gauge symmetry. The non universal $SU(3)_L \times U(1)_N$ symmetry in the lepton sector gives rise to non universal neutral and charged currents involving heavy non SM gauge bosons and SM leptons that yield radiative contributions to the $b \to s$, $b\to c$, $s\to u$ and $d\to u$ transitions arising from one loop level penguin and box diagrams. We found that the observables related to these transitions agree with their experimental values in a region of parameter space that includes TeV scale exotic up type quarks, within the LHC's reach.

==> Refflip1.tex <==
@article{Aaij_2016,
	author = "Aaij, R. and Abellán Beteta, C. and Adeva, B. and Adinolfi, M. and Affolder, A. and Ajaltouni, Z. and Akar, S. and Albrecht, J. and Alessio, F. and et al.",
	collaboration = "LHCb",
	title = "{Angular analysis of the $\text{B}^0 \rightarrow \text{K}^{*0}\mu^+ \mu^-$ decay using $3 \text{fb}^{-1}$ of intergrated luminosity}",
	eprint = "1512.04442",
	archivePrefix = "arXiv",
	primaryClass = "hep-ex",
	doi = "10.1007/jhep02(2016)104",
	journal = "JHEP",
	volume = "2016",
	number = "2",
	pages = "104",
	year = "2016"
}
@article{Aaboud_2018,
	author = "Aaboud, M. and Aad, G. and Abbott, B. and Abdinov, O. and Abeloos, B. and Abidi, S. H. and AbouZeid, O. S. and Abraham, N. L. and Abramowicz, H. and et al.",
	collaboration = "ATLAS",
	title = "{Angular analysis of $\text{B}_d^0 \rightarrow \text{K}^* \mu^+ \mu^-$ decays in \text{pp} collisions at $\sqrt{\text{s}}=8$ TeV with the ATLAS detector}",
	eprint = "1805.04000",
	archivePrefix = "arXiv",
	primaryClass = "hep-ex",
	doi = "10.1007/jhep10(2018)047",
	journal = "JHEP",
	volume = "2018",
	number = "10",
	pages = "047",
	year = "2018"
}
@article{Aubert_2006,
	author = "Aubert, B. and Barate, R. and Bona, M. and Boutigny, D. and Couderc, F. and Karyotakis, Y. and Lees, J. P. and Poireau, V. and Tisserand, V. and Zghiche, A. and et al.",
	collaboration = "BABAR",
	title = "{Measurements of branching fractions, rate asymmetries, and angular distributions in the rare 
	decays $\text{B} \rightarrow \text{K} \text{l}^+ \text{l}^-$ and $\text{B} \rightarrow \text{K}^* \text{l}^+ \text{l}^- $}",
	eprint = "0604007",
	archivePrefix = "arXiv",
	primaryClass = "hep-ex",
	doi = "10.1103/physrevd.73.092001",
	journal = "Phys. Rev. D",
	volume = "73",
	number = "18",
	pages = "092001",
	year = "2006"
}
@article{Lees_2016,
	author = "Lees, J. P. and Poireau, V. and Tisserand, V. and Grauges, E. and Palano, A. and Eigen, G. and Stugu, B. and Brown, D. N. and Kerth, L. T. and Kolomensky, Yu. G. and et al.",
	collaboration = "BABAR",
	title = "{Measurements of Angular Asymmetries in the Decay
	decays $\text{B} \rightarrow \text{K}^* \text{l}^+ \text{l}^-$}",
	eprint = "1508.07960",
	archivePrefix = "arXiv",
	primaryClass = "hep-ex",
	doi = "10.1103/physrevd.93.052015",
	journal = "Phys. Rev. D",
	volume = "93",
	number = "5",
	pages = "052015",
	year = "2016"
}
@article{Wei_2009,
	author = "Wei, J.-T. and Chang, P. and Adachi, I. and Aihara, H. and Aulchenko, V. and Aushev, T. and Bakich, A. M. and Balagura, V. and Barberio, E. and Bondar, A. and et al.",
	collaboration = "Belle",
	title = "{Measurements of the Differential Branching Fraction and Forward-Backward  Asymmetry for 
	$\text{B} \rightarrow \text{K}^* \text{l}^+ \text{l}^-$}",
	eprint = "0904.0770",
	archivePrefix = "arXiv",
	primaryClass = "hep-ex",
	doi = "10.1103/PhysRevLett.103.171801",
	journal = "Phys. Rev. Lett",
	volume = "103",
	number = "17",
	pages = "171801",
	year = "2009"
}

@article{bellecollaboration2016leptonflavordependent,
	author = "S. Wehle and C. Niebuhr and S. Yashchenko and I. Adachi and H. Aihara and S. Al Said and D. M. Asner and V. Aulchenko and T. Aushev and et al.",
	collaboration = "Belle",
	title = "{Lepton-Flavor-Dependent Angular Analysis of $\text{B} \rightarrow \text{K}^* \text{l}^+ \text{l}^-$}",
	eprint = "1612.05014",
	archivePrefix = "arXiv",
	primaryClass = "hep-ex",
	doi= "10.1103/PhysRevLett.118.111801",
	journal = "Phys. Rev. Lett.",
	volume = "118",
	number = "11",
	pages = "111801",
	year = "2017"
}
@article{Aaltonen_2012,
	author = "Aaltonen, T. and Álvarez González, B. and Amerio, S. and Amidei, D. and Anastassov, A. and Annovi, A. and Antos, J. and Apollinari, G. and Appel, J. A. and Apresyan, A. and et al.",
	collaboration = "CDF",
	title = "{Measurements of Angular Distributions in the Decays at $\text{B} \rightarrow \text{K}^* \text{l}^+ \text{l}^-$ CDF}",
	eprint = "1108.0695",
	archivePrefix = "arXiv",
	primaryClass = "hep-ex",
	doi= "10.1103/PhysRevLett.108.081807",
	journal = "Phys. Rev. Lett.",
	volume = "108",
	number = "8",
	pages = "081807",
	year = "2012"
}
@article{Aaij:2012vr,
	author = "Aaij, R. and Beteta, C. Abellan and Adametz, A. and Adeva, B. and Adinolfi, M. and Adrover, C. and Affolder, A. and Ajaltouni, Z. and Albrecht, J. and et al.",
	collaboration = "LHCb",
	title = "{Differential branching fraction and angular analysis of the $B^{+} \rightarrow K^{+}\mu^{+}\mu^{-}$ decay}",
	eprint = "1209.4284",
	archivePrefix = "arXiv",
	primaryClass = "hep-ex",
	doi= "10.1007/jhep02(2013)105",
	journal = "JHEP",
	volume = "1302",
	number = "2",
	pages = "105",
	year = "2013"
}
@article{Khachatryan_2016,
	author = "Khachatryan, V. and Sirunyan, A.M. and Tumasyan, A. and Adam, W. and Asilar, E. and Bergauer, T. and Brandstetter, J. and Brondolin, E. and Dragicevic, M. and Erö, J. and et al.",
	collaboration = "CMS",
	title = "{Angular analysis of the decay $\text{B}^0 \rightarrow \text{K}^{0*} \mu^+ \mu^-$ from \text{pp} collisions at $\sqrt{\text{s}}=8 \text{Tev}$}",
	eprint = "1507.08126",
	archivePrefix = "arXiv",
	primaryClass = "hep-ex",
	doi= "10.1016/j.physletb.2015.12.020",
	journal = "Phys. Lett.B",
	volume = "753",
	pages = "424",
	year = "2016"
}

@article{Sirunyan_2018,
	author = "Sirunyan, A.M. and Tumasyan, A. and Adam, W. and Ambrogi, F. and Asilar, E. and Bergauer, T. and Brandstetter, J. and Brondolin, E. and Dragicevic, M. and Erö, J. and et al.",
	collaboration = "CMS",
	title = "{Measurement of angular parameters from the decay $\text{B}^0 \rightarrow \text{K}^{0*} \mu^+ \mu^-$ in proton-proton collisions at $\sqrt{\text{s}}=8 \text{Tev}$}",
	eprint = "1710.02846",
	archivePrefix = "arXiv",
	primaryClass = "hep-ex",
	doi= "10.1016/j.physletb.2018.04.030",
	journal = "Phys. Lett.B",
	volume = "781",
	pages = "517",
	year = "2018"
}
@article{Aaij_2014,
	author = "Aaij, R. and Adeva, B. and Adinolfi, M. and Affolder, A. and Ajaltouni, Z. and Akar, S. and Albrecht, J. and Alessio, F. and Alexander, M. and Ali, S. and et al.",
	collaboration = "LHCb",
	title = "{Test of lepton universality using $\text{B}^+ \rightarrow \text{K}^{+} \text{l}^+ \text{l}^-$ decays}",
	eprint = "1406.6482",
	archivePrefix = "arXiv",
	primaryClass = "hep-ex",
	doi= "10.1103/PhysRevLett.113.151601",
	journal = "Phys. Rev. Lett",
	volume = "113",
	number ="15",
	pages = "151601",
	year = "2014"
}
@article{Aaij_2019,
	author = "Aaij, R. and Abellán Beteta, C. and Adeva, B. and Adinolfi, M. and Aidala, C. A. and Ajaltouni, Z. and Akar, S. and Albicocco, P. and Albrecht, J. and Alessio, F. and et al.",
	collaboration = "LHCb",
	title = "{Search for lepton-universality violation in $\text{B}^+ \rightarrow \text{K}^{+} \text{l}^+ \text{l}^-$ decays}",
	eprint = "1903.09252",
	archivePrefix = "arXiv",
	primaryClass = "hep-ex",
	doi= "10.1103/Phys.Rev.Lett.122.191801",
	journal = "Phys. Rev. Lett",
	volume = "122",
	number ="19",
	pages = "191801",
	year = "2019"
}
@article{Choudhury_2021,
	author = "Choudhury, S., Sandilya, S. et al.",
	collaboration = "Belle",
	title = "{Test of lepton flavor universality and search for lepton flavor violation in $\text{B} \rightarrow \text{K} \text{l}^+ \text{l}^-$ decays}",
	eprint = "1908.01848",
	archivePrefix = "arXiv",
	primaryClass = "hep-ex",
	doi= "10.1007/jhep03(2021)105",
	journal = "JHEP",
	volume = "2021",
	number ="3",
	pages = "105",
	year = "2021"
}
@article{Aaij2021,
	author = "R. Aaij and C. Abellán Beteta and T. Ackernley and B. Adeva and M. Adinolfi and H. Afsharnia and  et al.",
	collaboration = "LHCb",
	title = "{Test of lepton universality in beauty-quark decays}",
	eprint = "2103.11769",
	archivePrefix = "arXiv",
	primaryClass = "hep-ex",
	reportNumber = "LHCb-PAPER-2021-004, CERN-EP-2021-042",
	year = "2021"
}

@article{Bordone_2016,
	author = "Bordone, Marzia and Isidori, Gino and Pattori, Andrea",
	collaboration = "HFLAV",
	title = "{On the standard model predictions for $\text{R}_\text{K}, \text{R}_{\text{K}^*}$}",
	eprint = "1605.07633",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1140/epjc/s10052-016-4274-7",
	journal = "Eur. Phys. J. C",
	volume = "76",
	number = "8",
	pages = "440",
	year = "2016"
}
@article{straub2018flavio,
	author= "David M. Straub",
	title= "{flavio: a Python package for flavour and precision phenomenology in the Standard Model and beyond}", 
	year={2018},
	eprint= "1810.08132",
	archivePrefix= "arXiv",
	primaryClass= "hep-ph"
	
}

@article{Aaij_2017,
	author = "Aaij, R. and Adeva, B. and Adinolfi, M. and Ajaltouni, Z. and Akar, S. and Albrecht, J. and Alessio, F. and Alexander, M. and Ali, S. and et al.",
	collaboration = "LHCb",
	title = "{Test of lepton universality with $\text{B}^0 \rightarrow \text{K}^{0*}\text{l}^+ \text{l}^-$ decays}",
	eprint = "1705.05802",
	archivePrefix = "arXiv",
	primaryClass = "hep-ex",
	doi = "10.1007/jhep08(2017)055",
	journal = "JHEP",
	volume = "2017",
	number = "8",
	pages = "55",
	year = "2017"
}
@article{Wehle_2021,
	author = "Wehle, S. and Adachi, I. and Adamczyk, K. and Aihara, H. and Asner, D. M. and Atmacan, H. and Aulchenko, V. and Aushev, T. and Ayad, R. and Babu, V. and et al.",
	collaboration = "Belle",
	title = "{Test of lepton universality with $\text{B}^0 \rightarrow \text{K}^{0*}\text{l}^+ \text{l}^-$ in decays at Bell}",
	eprint = "1904.02440",
	archivePrefix = "arXiv",
	primaryClass = "hep-ex",
	doi = "10.1103/physrevlett.126.161801",
	journal = "Phys. Rev, Lett",
	volume = "126",
	number = "16",
	pages = "161801",
	year = "2021"
}
@article{Altmannshofer_2017,
	author = "Wolfgang Altmannshofer, Christoph Niehoff, Peter Stangl and David M. Straub",
	title = "{Status of the $\text{B}^0 \rightarrow \text{K}^{0*}\text{l}^+ \text{l}^-$ anomaly after Moriond 2017}",
	eprint = "1703.09189",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "	10.1140/epjc/s10052-017-4952-0",
	journal = "Eur. Phys. J. C",
	volume = "77",
	number = "6",
	pages = "377",
	year = "2017"
}

@article{Amhis:2019ckw,
	author = "Amhis, Y. and Banerjee, Sw. and Ben-Haim, E. and Bernlochner, F. U. and Bona, M. and Bozek, A. and Bozzi, C. and Brodzicka, J. and Chrzaszcz, M. and Dingfelder, J. and et al.",
	collaboration = "HFLAV",
	title = "{Averages of b-hadron, c-hadron, and $\tau $-lepton properties as of 2018}",
	eprint = "1909.12524",
	archivePrefix = "arXiv",
	primaryClass = "hep-ex",
	doi = "10.1140/epjc/s10052-020-8156-7",
	journal = "Eur. Phys. J. C",
	volume = "81",
	number = "3",
	pages = "226",
	year = "2021"
}

@article{Altmannshofer_2009,
	author = "Altmannshofer, Wolfgang and Ball, Patricia and Bharucha, Aoife and Buras, Andrzej J and Straub, David M and Wick, Michael",
	title = "{Symmetries and asymmetries of $\text{B} \rightarrow \text{K}\text{l}^+ \text{l}^-$ in the Standard Model and beyond}",
	eprint = "0811.1214",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1088/1126-6708/2009/01/019",
	journal = "JHEP",
	volume = "2009",
	number = "01",
	pages = "019",
	year = "2009"
}

@article{Bobeth_2012,
	author = "Bobeth, Christoph and Hiller, Gudrun and van Dyk, Danny and Wacker, Christian",
	title = "{The decay $\text{B} \rightarrow \text{K}\text{l}^+ \text{l}^-$ at low hadronic recoil and model-independent $\Delta B=1$ constraints}",
	eprint = "1111.2558",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/jhep01(2012)107",
	journal = "JHEP",
	volume = "2012",
	number = "01",
	pages = "107",
	year = "2012"
}
@article{Matias_2012,
	author = "Matias, J. and Mescia, F. and Ramon, M. and Virto, J.",
	title = "{Complete Anatomy of $\text{B} \rightarrow \text{K}^*\text{l}\text{l}$ and its angular distribution}",
	eprint = "1202.4266",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/jhep04(2012)104",
	journal = "JHEP",
	volume = "2012",
	number = "04",
	pages = "104",
	year = "2012"
}
@article{Descotes_Genon_2013,
	author = "Sebastien Descotes-Genon, Joaquim Matias, Marc Ramon, Javier Virto",
	title = "{Implications from clean observables for the binned analysis of $\text{B} \rightarrow \text{K}^*\text{l}\text{l}$ at large recoil}",
	eprint = "1207.2753",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "	10.1007/JHEP01(2013)048",
	journal = "JHEP",
	volume = "2013",
	number = "01",
	pages = "048",
	year = "2013"
}
@article{Matias_2014,
	author = "Joaquim Matias, Nicola Serra",
	title = "{Symmetry relations between angular observables in $\text{B} \rightarrow \text{K}^*\text{l}\text{l}$ and the LHCb $\textbf{P}_5$'anomaly}",
	eprint = "1402.6855",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "	10.1103/physrevd.90.034002",
	journal = "Phys. Rev. D",
	volume = "90",
	number = "3",
	pages = "034002",
	year = "2014"
}
@article{Khodjamirian_2010,
	author = "Joaquim Matias, Nicola Serra",
	title = "{Charm-loop effect in $\text{B} \rightarrow \text{K}^*\text{l}\text{l}$ and $\text{B} \rightarrow \text{K}^*\gamma$}",
	eprint = "1006.4945",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "	10.1007/JHEP09(2010)089",
	journal = "JHEP",
	volume = "2010",
	number = "9",
	pages = "089",
	year = "2010"
}
@article{Khodjamirian_2013,
	author = "Khodjamirian, A. and Mannel, Th. and Wang, Y.-M.",
	title = "{$\text{B} \rightarrow \text{K}^*\text{l}\text{l}$ decay at large hadronic recoil}",
	eprint = "1211.0234",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "	10.1007/JHEP02(2013)010",
	journal = "JHEP",
	volume = "2013",
	number = "2",
	pages = "010",
	year = "2013"
}
@article{lyon2014resonances,
	author = "A. Khodjiamirian, Th. Mannel, Y.-M.Wang",
	title = "{Resonances gone topsy turvy -the charm of QCD or new physics in $\text{b} \rightarrow \text{s}\text{l}^+\text{l}^-$ }",
	eprint = "1406.0566",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph"
}
@article{Descotes_Genon_2014,
	author = "S\'{e}bastien Descotes$-$Genon, Lars Hofer, Joaquim Matias, Javier Virto", 
	title = "{On the impact of power corrections in the prediction of  $\text{B} \to \text{K} \mu^+ \mu^-$ observables}",
	eprint = "1407.8526",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/jhep12(2014)125",
	journal = "JHEP",
	volume = "2014",
	number = "12",
	pages = "125",
	year = "2014"
}
@article{Capdevila_2017,
	author = "Bernat Capdevila, S\'{e}bastien Descotes$-$Genon, Lars Hofer, Joaquim Matias", 
	title = "{Hadronic uncertainties in $\text{B} \to \text{K} \mu^+ \mu^-$: a state of the art analysis}",
	eprint = "1701.08672",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/jhep04(2017)016",
	journal = "JHEP",
	volume = "2017",
	number = "4",
	pages = "016",
	year = "2017"
}
@article{Blake_2018,
	author = "Blake, T. and Egede, U. and Owen, P. and Petridis, K. A. and Pomery, G.", 
	title = "{An empirical model of the long-distance contributions to $\text{B} \to \text{K} \mu^+ \mu^-$ transitions}",
	eprint = "1709.03921",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "	10.1140/epjc/s10052-018-5937-3",
	journal = "JHEP",
	volume = "78",
	number = "6",
	pages = "453",
	year = "2018"
}
@article{Beneke:2017vpq,
	author = "Beneke, Martin and Bobeth, Christoph and Szafron, Robert",
	title = "{Enhanced electromagnetic correction to the rare $B$-meson decay $\text{B}_{\text{s,d}} \to \mu^+ \mu^-$}",
	eprint = "1708.09152",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	reportNumber = "TUM-HEP-1094-17",
	doi = "10.1103/PhysRevLett.120.011801",
	journal = "Phys. Rev. Lett.",
	volume = "120",
	number = "1",
	pages = "011801",
	year = "2018"
}
@article{Bobeth:2013uxa,
	author = "Bobeth, Christoph and Gorbahn, Martin and Hermann, Thomas and Misiak, Mikolaj and Stamou, Emmanuel and Steinhauser, Matthias",
	title = "{$\text{B}_{\text{s,d}} \to \text{l}^+ \text{l}^-$ in the Standard Model with Reduced Theoretical Uncertainty}",
	eprint = "1311.0903",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	reportNumber = "FLAVOUR(267104)-ERC-53, LTH-990, SFB-CPP-13-82, TTP13-033",
	doi = "10.1103/PhysRevLett.112.101801",
	journal = "Phys. Rev. Lett.",
	volume = "112",
	number = "10",
	pages = "101801",
	year = "2014"
}

@article{Altmannshofer:2013foa,
	author = "Altmannshofer, Wolfgang and Straub, David M.",
	title = "{New Physics in $\text{B} \to \text{K}^*\mu\mu$?}",
	eprint = "1308.1501",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	reportNumber = "FERMILAB-PUB-13-310-T, MITP-13-047",
	doi = "10.1140/epjc/s10052-013-2646-9",
	journal = "Eur. Phys. J. C",
	volume = "73",
	number = "12",
	pages = "2646",
	year = "2013"
}
@article{Descotes-Genon:2015uva,
	author = "Descotes-Genon, S\'ebastien and Hofer, Lars and Matias, Joaquim and Virto, Javier",
	title = "{Global analysis of $\text{b}\to \text{s}\text{ll}$ anomalies}",
	eprint = "1510.04239",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	reportNumber = "LPT-ORSAY-15-68, QFET-2015-29, SI-HEP-2015-19",
	doi = "10.1007/JHEP06(2016)092",
	journal = "JHEP",
	volume = "2016",
	number = "6"
	pages = "092",
	year = "2016"
}
@article{Altmannshofer2015,
	author = "Altmannshofer, Wolfgang and Straub, David M.",
	title = "{New physics in $\text{b} \rightarrow \text{s}$ transitions after LHC run 1}",
	eprint = "1411.3161",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	reportNumber = "LPT-ORSAY-15-68, QFET-2015-29, SI-HEP-2015-19",
	doi = "10.1140/epjc/s10052-015-3602-7",
	journal = "Eur. Phys. J. C",
	volume = "75",
	pages = "382",
	number = "8",
	year = "2015"
}
@article{pdg2020,
	author = "Zyla et al. (Particle Data Group), P.A",
	title = "{Review of Particle Physics}",
	primaryClass = "hep-ph",
	reportNumber = "LPT-ORSAY-15-68, QFET-2015-29, SI-HEP-2015-19",
	doi = "10.1093/ptep/ptaa104",
	journal = "Prog. Theor. Exp. Phys",
	volume = "2020",
	pages = "8",
	year = "2020"
}
@article{Hiller_2004,
	author = "Hiller, Gudrun and Kruger, Frank",
	title = "{More Model-Independent Analysis of $\text{b} \rightarrow \text{s}$ Processes}",
	eprint = "0310219",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1103/physrevd.69.074020",
	journal = "Phys. Rev. D",
	volume = "79",
	pages = "69.074020",
	number = "7",
	year = "2014"
}
@article{Hiller_2015,
	author = "Hiller, Gudrun and Kruger, Frank",
	title = "{Diagnosing lepton-nonuniverality $\text{b} \rightarrow \text{s}\text{ll}$ }",
	eprint = "1411.4773",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/JHEP02(2015)055",
	journal = "JHEP",
	volume = "2015",
	pages = "055",
	number = "2",
	year = "2015"
}
@article{Altmannshofer_2017a,
	author = "Altmannshofer, Wolfgang and Stangl, Peter and Straub, David M.",
	title = "{Interpreting hints for lepton flavor universality violation }",
	eprint = "1704.05435",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1103/physrevd.96.055008",
	journal = "Phys. Rev. D",
	volume = "96",
	pages = "055008",
	number = "5",
	year = "2017"
}
@article{Arbey_2019,
	author = "Arbey, A. and Hurth, T. and Mahmoudi, F. and Martínez Santos, D. and Neshatpour, S.",
	title = "{Update on the $\text{b} \to \text{s}$ anormalies}",
	eprint = "1904.08399",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1103/physrevd.100.015045",
	journal = "Phys. Rev. D",
	volume = "100",
	pages = "015045",
	number = "1",
	year = "2019"
}
@article{Alok_2019,
	author = "Arbey, A. and Hurth, T. and Mahmoudi, F. and Martínez Santos, D. and Neshatpour, S.",
	title = "{Continuing search for new physics in $\text{b} \to \text{s} \mu^+ \mu^-$ decays: two operators at a time }",
	eprint = "1903.09617",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/jhep06(2019)089",
	journal = "JHEP",
	volume = "2019",
	pages = "089",
	number = "06",
	year = "2019"
}
@article{altmannshofer2021new,
	author = "Wolfgang Altmannshofer and Peter Stangl",
	title = "{New physics in rare $\text{B}$ decays after Moriond 2021 }",
	eprint = "2103.13370",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph"
	year = "2021"
	}
@article{hurth2021indications,
	author = "Arbey, A. and Hurth, T. and Mahmoudi, F. and Martínez Santos, D. and Neshatpour, S.",
	title = "{More indicatión for lepton nonuniversality  $\text{b} \to \text{s} \text{l}^+ \text{l}^-$}",
	eprint = "2104.10058",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	year = "2021"
}
@article{Allanach_2016,
	author = "Allanach, Ben and Queiroz, Farinaldo S. and Strumia, Alessandro and Sun, Sichun",
	title = "{$\text{Z}^\prime$ models for the LHCb and $\text{g}−2$ muon anomalies }",
	eprint = "1511.07447",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1103/physrevd.93.055045",
	journal = "Phys. Rev. D",
	volume = "93",
	pages = "055045",
	number = "5",
	year = "2016"
}
@article{Altmannshofer_2016,
	author = "Altmannshofer, Wolfgang and Gori, Stefania and Profumo, Stefano and Queiroz, Farinaldo S.",
	title = "{Explaining dark matter and \text{B} decay anomalies with an $\text{L}_\mu -\text{L}_\tau$ model}",
	eprint = "1609.04026",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/jhep12(2016)106",
	journal = "JHEP",
	volume = "2016",
	pages = "106",
	number = "12",
	year = "2016"
}
@article{gripaios2015composite,
	author = "Ben Gripaios, Marco Nardecchia, S. A. Renner",
	title = "{Composite leptoquarks and anomalies in $B$-meson decays}",
	eprint = "1412.1791",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/JHEP05(2015)065",
	journal = "JHEP",
	volume = "2015",
	pages = "065",
	number = "05",
	year = "2015"
}
@article{Fajfer_2016,
	author = "S. Fajfer and N. Ko\v{s}nik",
    title = "Vector leptoquark resolution of $\text{R}_\text{K}$ and $\text{R}_{\text{D}^*} puzzles $",
	eprint = "1511.06024",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1016/j.physletb.2016.02.018",
	journal = "Phys. Lett. B",
	volume = "46",
	pages = "270",
	number = "10",
	year = "2016"
}
@article{Pisano_1992,
	author = "Pisano, F. and Pleitez, V.",
	title = "$\text{SU(3)}\times \text{U(1)}$ model for electroweak interactions",
	eprint = "9206242",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "	10.1103/PhysRevD.46.410",
	journal = "Phys. Rev. D",
	volume = "46",
	pages = "410",
	number = "1",
	year = "1992"
}
@article{PhysRevLett.69.2889,
author = "P. H. Frampton",
title = "Chiral dilepton model and the flavor question ",
doi = "10.1103/PhysRevLett.69.2889",
journal = "Phys. Rev. Lett",
volume = "69",
pages = "2889",
year = "1992"
}
@article{PhysRevD.47.4158,
	author = "Foot, R. and Hern\'andez, O. F. and Pisano, F. and Pleitez, V.",
	title = "Lepton masses in an $\text{SU(3)}_\text{L}\times \text{U(1)}_\text{N}$ gauge model",
	eprint = "9207264",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "	10.1103/physrevd.47.4158",
	journal = "Phys. Rev. D",
	volume = "47",
	pages = "4158",
	number = "9",
	year = "1993"
}
@article{PhysRevD.22.738,
	author = "Foot, R. and Hern\'andez, O. F. and Pisano, F. and Pleitez, V.",
	title = "Canonical neutral-current predictions from the weak-electromagnetic 
	gauge group $\text{SU(3)}\times \text{U(1)}$ ",
	doi = "	10.1103/physrevd.47.4158",
	journal = "Phys. Rev. D",
	volume = "22",
	pages = "738",
	number = "0",
	year = "1980"
}
@article{Montero_1993,
	author = "Montero, J. C. and Pisano, F. and Pleitez, V.",
	title = "Neutral currents and Glashow-Iliopoulos-Maiani mechanism in $\text{SU(3)}_\text{L}\times \text{U(1)}_\text{N}$ models for electroweak interactions",
	eprint = "9212271",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "	10.1103/PhysRevD.47.2918",
	journal = "Phys. Rev. D",
	volume = "47",
	pages = "2918",
	number = "7",
	year = "1993"
}
@article{Foot_1994,
	author = "Foot, Robert and Long, Hoang Ngoc and Tran, Tuan A.",
	title = "$\text{SU(3)}_\text{L}\times \text{U(1)}_\text{N}$ and $\text{SU(4)}_\text{L}\times \text{U(1)}_\text{N}$ gauge models with right-handed neutrinos",
	eprint = "9402243",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "	10.1103/PhysRevD.50.R34",
	journal = "Phys. Rev. D",
	volume = "50",
	pages = "R34",
	number = "1",
	year = "1994"
}

@article{Buras_2014,
	title={331 models facing new b → sμ + μ − data},
	volume={2014},
	ISSN={1029-8479},
	url={http://dx.doi.org/10.1007/JHEP02(2014)112},
	DOI={10.1007/jhep02(2014)112},
	number={2},
	journal={Journal of High Energy Physics},
	publisher={Springer Science and Business Media LLC},
	author={Buras, Andrzej J. and De Fazio, Fulvia and Girrbach, Jennifer},
	year={2014},
	month={Feb}
}

@article{Buras_2014A,
	author = "Andrzej J. Buras, Fulvia De Fazio, Jennifer Girrbach",
	title = "$\text{331}$ models facing new $\text{b}\to\text{s} \mu^+ \mu^-$ data",
	eprint = "1311.6729",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "	10.1007/JHEP02(2014)112",
	journal = "JHEP",
	volume = "2014",
	pages = "112",
	number = "2",
	year = "2014"
}
@article{Buras_2013,
	author = "Buras, Andrzej J. and De Fazio, Fulvia and Girrbach, Jennifer and Carlucci, Maria V.",
	title = "The anatomy of quark flavour observables in 331 models in the flavour precision era",
	eprint = "1211.1237",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "	10.1007/jhep02(2013)023",
	journal = "JHEP",
	volume = "2013",
	pages = "023",
	number = "02",
	year = "2013"
}
@article{Gauld_2014,
	author = "Gauld, Rhorry and Goertz, Florian and Haisch, Ulrich",
	title = "An explicit $\text{Z}^\prime$ boson explanation of the $\text{B} \rightarrow \text{K}^* \mu^+ \mu^-$ anomaly",
	eprint = "1310.1082",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "	10.1007/JHEP01(2014)069",
	journal = "JHEP",
	volume = "2014",
	pages = "069",
	number = "01",
	year = "2014"
}
@article{Buras_2016,
	author = "Buras, Andrzej J. and De Fazio, Fulvia",
	title = "$\varepsilon^\prime /\varepsilon$ in 331 models",
	eprint = "1512.02869",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "	10.1007/jhep03(2016)010",
	journal = "JHEP",
	volume = "2016",
	pages = "010",
	number = "3",
	year = "2016"
}
@article{Fonseca_2016,
	author = "Fonseca, Renato M. and Hirsch, Martin",
	title = "A flipped 331 model",
	eprint = "1606.01109",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "	10.1007/jhep08(2016)003",
	journal = "JHEP",
	volume = "2016",
	pages = "003",
	number = "8",
	year = "2016"
}
@article{Huong_2019,
	author = "Huong, D.T. and Dinh, D.N. and Thien, L.D. and Van Dong, Phung",
	title = "Dark matter and flavor changing in the flipped 3-3-1 model",
	eprint = "1906.05240",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "	10.1007/JHEP08(2019)051",
	journal = "JHEP",
	volume = "2019",
	pages = "051",
	number = "8",
	year = "2019"
}
@article{Van_Loi_2020,
	author = "Van Loi, Duong and Van Dong, Phung and Van Soa, Dang",
	title = "Neutrino mass and dark matter from an approximate $\text{B}-\text{L}$ symmetry",
	eprint = "1911.04902",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/JHEP05(2020)090",
	journal = "JHEP",
	volume = "2020",
	pages = "090",
	number = "5",
	year = "2020"
}
@article{PhysRevLett.114.221801,
	author = "Misiak, M. and Asatrian, H. M. and Boughezal, R. and Czakon, M. and Ewerth, T. and Ferroglia, A. and Fiedler, P. and Gambino, P. and Greub, C. and Haisch, U. and Huber, T. and Kami\ifmmode \acute{n}\else \'{n}\fi{}ski, M. and Ossola, G. and Poradzi\ifmmode \acute{n}\else \'{n}\fi{}ski, M. and Rehman, A. and Schutzmeier, T. and Steinhauser, M. and Virto, J.",
	title = "Updated Next-to-Next-to-Leading-Order QCD Predictions for the Weak Radiative $B$-Meson Decays",
	eprint = "1503.01789",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1103/PhysRevLett.114.221801",
	journal = "Phys. Rev. Lett.",
	volume = "114",
	pages = "221801",
	number = "5",
	year = "2015"
}
@article{Blanke_2012,
	author = "Blanke, Monika and Buras, Andrzej J. and Gemmler, Katrin and Heidsieck, Tillmann",
	title = "$\Delta F = 2$ observables and $\text{B} \rightarrow \text{X}_\text{q} \ga$ decays in the left-right model: Higgs particles striking back",
	eprint = "1111.5014",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/JHEP03(2012)024",
	journal = "JHEP",
	volume = "2012",
	pages = "024",
	number = "3",
	year = "2012"
}
@article{duy2021physical,
	author = "N. T. Duy and Takeo Inami and D. T. Huong",
	title = "Physical constraints derived from FCNC in the $\text{3-3-1-1}$ model",
	eprint = "1111.5014",
	archivePrefix = "arXiv",
	primaryClass = "hep-ph",
	doi = "10.1007/JHEP03(2012)024",
	journal = "JHEP",
	volume = "2012",
	pages = "024",
	number = "3",
	year = "2012"
}

